NoPe-NeRF: Optimising Neural Radiance Field with No Pose Prior

Training a Neural Radiance Field (NeRF) without pre-computed camera poses is challenging. Recent advances in this direction demonstrate the possibility of jointly optimising a NeRF and camera poses in forward-facing scenes. However, these methods still face difficulties during dramatic camera movement. We tackle this challenging problem by incorporating undistorted monocular depth priors. These priors are generated by correcting scale and shift parameters during training, with which we are then able to constrain the relative poses between consecutive frames. This constraint is achieved using our proposed novel loss functions. Experiments on real-world indoor and outdoor scenes show that our method can handle challenging camera trajectories and outperforms existing methods in terms of novel view rendering quality and pose estimation accuracy. Our project page is https://nope-nerf.active.vision.

==> 01_intro.tex <==
\section{Introduction} \label{sec:intro}
Photo-realistic reconstruction of a scene from a stream of RGB images requires both an accurate 3D geometry reconstruction and view-dependent appearance modelling that is a function of the light source and surface material.
Recently, Neural Radiance Fields (NeRF)~\cite{mildenhall2021nerf} has shown high-quality results for generating photo-realistic images from novel viewpoints given a sparse set of images. 
% The key to NeRF is the continuous implicit representation that maps each 3D point (and viewing direction) to the corresponding geometry and appearance properties.
To train a NeRF model,
accurate camera pose registration for the captured images is necessary,
and it was often approached by using COLMAP~\cite{schonberger2016structure}, a state-of-the-art structure-from-motion (SfM) system.
However, in challenging real-world scenarios, particularly low-texture scenes, SfM methods often fail to find reliable correspondences and result in inaccurate or unsuccessful camera pose estimation. 
Furthermore, SfM is not an end-to-end trainable system, which leads to a two-stage process for NeRF optimisation.
% with a time complexity of $O(N^4)$~\cite{wu2013towards} ($N$ denotes image numbers),
% the computation time of SfM systems increases significantly with input frame numbers.

Reconstructing scene geometry and estimating camera pose is a ``chicken-and-egg" problem in computer vision.
The classic algorithm to address them often uses a bundle adjustment framework~\cite{triggs1999bundle},
where two parts are jointly optimised.
Inspired by it, recent works such as NeRFmm~\cite{wang2021nerfmm} and BARF~\cite{lin2021barf} simultaneously optimised camera poses and implicit scene representation,
and they showcased equivalent results with the original NeRF that uses COLMAP poses.
However, we find that accurate results are only shown in forward-facing scenes,
and these methods indeed do not work well in more challenging scenarios,
\eg, a casual object scanning using a handheld camera.
As discussed in the recent SC-DepthV2~\cite{bian2021auto},
the main challenge in casual video scanning is the large camera rotation that prevents neural networks from learning accurate scene geometry.
We conjecture that existing methods are confronted by the same issue and are easy to fall into local minima due to the lack of good pose initialisation.
% This is because the poses are optimised iteratively without a good initialization, and hence are easily fall into local minimums.

% % \kejie{NeRF's problem: Pose and geometry constraint -> realise deep-learnt depth prior can be the solution -> what is the problem of using depth naively -> so our method...}
% NeRF has two limitations. First, the camera calibration is done externally as a preprocessing step using packages like COLMAP~\cite{schonberger2016structure}. 
% The decoupling of camera parameters estimation and NeRF training is sub-optimal as the errors introduced in one component would be propagated to the rest of the pipeline. Although some following works~\cite{wang2021nerfmm, lin2021barf} propose to optimise NeRF with unknown poses, but as local registration algorithms, they are generally not robust for camera poses with large rotation. The second problem of NeRF is that the geometry reconstructed can be incorrect when there are no sufficient input frames. 

% In this paper, we propose \methodname to tackle these two problems simultaneously by introducing a depth prior learned from a mono-depth estimation network. On the one hand, as a direct supervision, it provides stronger geometric constraint for surfaces. On the other hand, the point clouds reconstructed from the mono-depth maps can be used to optimise the relative poses between frames. Due to the inherent ambiguity of monocular vision, the mono-depth maps can have different distortions, which lead to erroneous result if using them directly. Therefore, our main challenge of is to recover the distortion of each depth map to improve the utilisability and thus make better pose estimation and NeRF optimisation jointly.
% Following works such as NeRFmm~\cite{wang2021nerfmm} and BARF~\cite{lin2021barf} show that camera parameters can be jointly optimised together with the implicit 3D scene representation. 
% Although these methods works well on forward facing scenes, they are
% Additionally, NeRF also has ambiguity in texture-less areas, which not only effects the geometry reconstructed, but also makes pose estimation more difficult.

In this paper, we propose \methodname that jointly optimises camera parameters and 3D scene representation from a casually captured video of objects.
The key insight of \methodname, which allows us to circumvent the limitation of previous works~\cite{wang2021nerfmm, lin2021barf, jeong2021self}, is improving NeRF-based global pose estimation by adding effective local pairwise pose constraints.
This is approached by leveraging an off-the-shelf mono-depth estimation network and our proposed scale-shift-invariant pairwise losses.
Specifically, as the predicted depth by the mono-depth estimation network is often distorted in an unknown scale and shift, which limits their use in 3D reconstruction,
we propose to jointly recover their distortion parameters with NeRF.
In this way, the recovered depth map enables us to constrain both pairwise relative pose optimization and NeRF by regularizing its rendered depth.
As a result, our proposed method significantly boosts the robustness of NeRF optimisation from challenging object-scanning videos.


In summary, our contributions include
\begin{itemize}
% \item Provide geometric constraints to NeRF optimisation by formulating the distortion for each depth map.
% \item Introduce a novel ICP-inspired loss to optimise the relative poses with the mono-depth maps and merge into the NeRF model with pose optimisation to offer better pose estimation together.
% \item Achieve better performance in terms of pose accuracy, depth accuracy and view synthesis quality in various scenes, including those where other methods fail.

% \item Add  geometric constraint to NeRF optimisation and optimise poses using the point cloud reconstructed from the depth maps.
% \item Parameterise the distortions of depth maps and optimise jointly with NeRF to gain multi-view consistency.
% \item Successfully reconstruct various scenes with complex trajectories, including those where other methods fail.

\item We propose \methodname that robustly optimises a NeRF model without the requirement of pre-computed poses in a casual object scanning video.

% \item We propose scale-shift-invariant pairwise losses, which work with an off-the-shelf mono-depth estimation network for constraining relative camera pose optimisation.
\item We propose to use mono-depth estimation, which is undistorted in our framework to provide both local and global constraints to optimise NeRF.

\item The proposed method outperforms the previous alternatives by a significant margin. Furthermore, our method generally achieves on-par performance with the COLMAP+NeRF pipeline and significantly beats the latter in challenging low-texture scenes.

\end{itemize}
% The remainder of the paper is structured as follows: After a review of related works in \cref{sec:related}, we present our method in \cref{sec:method} and show qualitative and quantitative results in \cref{sec:exp}. Finally, we conclude in \cref{sec:conclu}.

==> 01_intro_v1.tex <==
\section{Introduction} \label{sec:intro}
Given a video or several consecutive images of a scene, humans can easily make reasonable reasoning about the 3D geometry and colour of the scene as well as the position and orientation of the camera. 
The inference depends on both the observed scene as well as the general prior knowledge gained by human from previous observations. In traditional computer vision, the problem of recovering the 3D scene and camera poses can be solved using structure from motion (SfM) \cite{hartley2003multiple} or simultaneous localization and mapping (SLAM) \cite{mur2015orb}. 
However, these methods require computationally expensive feature matching, and rely on good texture and change in viewpoints. 
Moreover, the none-differentiable nature and the output form (point clouds) limit their ability to be combined with other upstream or downstream vision tasks.

Recently, Neural Radiance Fields (NeRF)~\cite{mildenhall2021nerf} has been widely applied in vision tasks. 
By representing 3D scenes as a continuous function mapping each 3D point to its geometry and appearance representations, we are able to synthesise photo-realistic novel views with an arbitrary resolution. Following works such as NeRFmm~\cite{wang2021nerfmm} and BARF~\cite{lin2021barf} show that camera parameters can be jointly optimised with the 3D scene representation, hence provides an alternative to traditional geometric-based approaches. 
Although these methods works well on forward facing scenes, they are generally not robust for camera poses with large rotation and are easily fall into local minimums. 
Additionally, NeRF also has ambiguity in texture-less areas, which not only effects the geometry reconstructed, but also makes pose estimation more difficult.

An alternative way for pose estimation is estimating the relative poses between frames using Iterative Closest Point (ICP). 
Traditional ICP algorithms can handle point clouds with the same scale or up to a scale factor. 
It cannot handle distorted point clouds, (i.e. unprojected depth map from a monocular network). 
However, comparing with obtaining real point clouds/depths using sensors, pseudo depth maps are easier to be accessed from a pre-trained depth estimation model. 

We propose an algorithm to make use of pseudo depth maps to boost pose optimisation with NeRF in two ways. 
First, as a direct supervision, it provides stronger geometric constraint for surfaces. 
Second, we use the point clouds reconstructed from pseudo depth maps to optimise the relative poses between frames and the distortion of depth maps. 
By sharing the parameters with NeRF, we are able to learn multi-view consistent distortions and obtain better pose estimation and NeRF reconstruction.

In summary, by introducing monocular depth estimations as input, we:
\begin{itemize}
\item Provide geometric constraints to NeRF optimisation by formulating the distortion for each depth map.
\item Introduce a novel ICP-inspired loss to optimise the relative poses with the pseudo depth maps and merge into the NeRF model with pose optimisation to offer better pose estimation together.
\item Achieve better performance in terms of pose accuracy, depth accuracy and view synthesis quality in various scenes, including those where other methods fail.
\end{itemize}


==> 01_intro_v2.tex <==
\section{Introduction} \label{sec:intro}
Photo-realistic reconstruction of a scene from a stream of RGB images requires both an accurate 3D geometry reconstruction and view-dependent appearance modelling that is a function of light source and surface material.
Recently, Neural Radiance Fields (NeRF)~\cite{mildenhall2021nerf} has shown impressive results on generating photo-realistic images from novel viewpoints given a sparse set of images. 
The key to NeRF is the continuous implicit representation that maps each 3D point (and viewing direction) to the corresponding geometry and appearance properties.

% \kejie{NeRF's problem: Pose and geometry constraint -> realize deep-learnt depth prior can be the solution -> what is the problem of using depth naively -> so our method...}
NeRF has two limitations. First, the camera calibration is done externally as a preprocessing step using packages like COLMAP~\cite{schonberger2016structure}. 
The decoupling of camera parameters estimation and NeRF training is sub-optimal as the errors introduced in one component would be propagated to the rest of the pipeline. Although some following works~\cite{wang2021nerfmm, lin2021barf} propose to optimise NeRF with unknown poses, but as local registration algorithms, they are generally not robust for camera poses with large rotation. The second problem of NeRF is that the geometry reconstructed can be incorrect when there are no sufficient input frames. 

In this paper, we propose \methodname to tackle these two problems simultaneously by introducing a depth prior learned from a monocular depth estimation network. On the one hand, as a direct supervision, it provides stronger geometric constraint for surfaces. On the other hand, the point clouds reconstructed from the pseudo depth maps can be used to optimise the relative poses between frames. Due to the inherent ambiguity of monocular vision, the pseudo depth maps can have different distortions, which lead to erroneous result if using them directly. Therefore, our main challenge of is to recover the distortion of each depth map to improve the utilisability and thus make better pose estimation and NeRF optimisation jointly.

In summary, by introducing monocular depth estimations as input as input, we:
\begin{itemize}
% \item Provide geometric constraints to NeRF optimisation by formulating the distortion for each depth map.
% \item Introduce a novel ICP-inspired loss to optimise the relative poses with the pseudo depth maps and merge into the NeRF model with pose optimisation to offer better pose estimation together.
% \item Achieve better performance in terms of pose accuracy, depth accuracy and view synthesis quality in various scenes, including those where other methods fail.
\item Add  geometric constraint to NeRF optimisation and optimise poses using the point cloud reconstructed from the depth maps.
\item Parameterise the distortions of depth maps and optimise jointly with NeRF to gain multi-view consistency.
\item Successfully reconstruct various scenes with complex trajectories, including those where other methods fail.

\end{itemize}


==> 03_preliminary.tex <==
% \vspace{-0.6cm}
\section{Preliminary} \label{sec:preliminary}



==> 04_method.tex <==
\begin{figure*}[ht]
    \centering
    \includegraphics[width=\linewidth]{images/icp_nerfmm.pdf}
    \caption{\textbf{Model Overview.}
    Our method takes a sequence of images as input to reconstruct NeRF and jointly estimates the camera poses of the frames. We first generate mono-depths from a mono-depth estimation network and reconstruct the point clouds. We then optimise NeRF, camera poses and depth distortion parameters jointly with inter-frame and NeRF losses.
    % Given a sequence of images and the point clouds reconstructed from their mono-depth estimations, we optimise the camera poses $\left\{\mathbf{T}_{i}\right\}_{i=0}^{N-1}$, NeRF model $F_\theta$ and depth distortion parameters $\left\{(\alpha_i, \beta_i) \right\}_{i=0}^{N-1}$ jointly. 
    % For frame $I_i$, we select a reference frame $I_j$ ($I_{i+1}$ in this example) and compute the pairwise losses of the point clouds while recovering their distortions. Meanwhile, we optimise a NeRF model with RGB and depth supervision to reconstruct the 3D scene and constrain the camera poses and distortion parameters globally.
    }
    \label{fig:model}
\end{figure*}

\section{Method}\label{sec:method}
% \zirui{I don't think local and glabal are accurate terms here. Both nerfmm and barf only update individual images each time. \textit{Global} to me refers more like Global BA, where everything is connected. If it's me to separate levels, I would say nerfmm/barf is doing individual image level optimisation (very local), nope-nerf is doing inter-frame level optimisation (between local and global), and COLMAP is doing the entire graph optimisation (global).}

We present \methodname, an end-to-end differentiable method for joint pose estimation and novel view synthesis, given a video with known camera intrinsics.
The key to our method is a robust optimisation of camera rotation in challenging scenes,
where most existing pose-unknown NeRF methods~\cite{lin2021barf, wang2021nerfmm, jeong2021self} often fail.
To achieve this, we introduce single-image depth priors from a pre-trained mono-depth estimation network,
based on which we propose effective constraints on relative camera poses and scene geometry.
However, as mono-depth is distorted by unknown scales and shifts,
it is non-trivial to use. 
We propose to jointly learn the distortion parameters for each depth map in the overall optimisation.

In the following subsections, we go over the NeRF model and NeRF optimisation with unknown poses in \cref{sec: nerf} and \cref{sec: nerfmm} respectively. 
In \cref{sec: nop-nerf}, we show how to constrain relative poses and geometry with mono-depth. 
We discuss how to parameterise distorted depth maps into the unknown-pose NeRF model and introduce an inter-frame point cloud loss for relative pose estimation. 
Finally, we build \methodname that jointly optimises poses, depth distortions and 3D representation of the scene, 
which achieves robust optimisation of complex pose trajectories. 
An overview of our method is shown in \cref{fig:model}.

\subsection{Neural Radiance Field} \label{sec: nerf}

Neural Radiance Field (NeRF)~\cite{mildenhall2021nerf} represents the scene as a mapping $F_\Theta: (\mathbf{x}, \mathbf{d}) \rightarrow (\mathbf{c}, \sigma)$, 
which maps a 3D location $x \in \mathbb{R}^3$ and viewing direction $\mathbf{d} \in \mathbb{R}^3$ to radiance colour $\mathbf{c} \in \mathbb{R}^3$ and volume density $\sigma$.
Given RGB images $\mathcal{I} = \left\{I_{i} \mid i=0 \ldots N-1 \right\}$ of a scene with their camera poses $\Pi = \{\pi_{i} \mid i=0 \ldots N-1\}$,
% learns an implicit representation of a scene from the captured RGB images $\mathcal{I} = \left\{I_{i} \mid i=0 \ldots N-1 \right\}$ of that,
% where accurate camera poses $\Pi = \{\pi_{i} \mid i=0 \ldots N-1\}$ are assumed to be known.
% Given consecutive RGB images of a scene $\mathcal{I} = \left\{I_{i} \mid i=0 \ldots N-1 \right\}$ and their camera poses $\Pi = \{\pi_{i} \mid i=0 \ldots N-1\}$, Neural Radiance Field (NeRF)~\cite{mildenhall2021nerf} learns an implicit representation of the scene including both appearance and geometry. 
NeRF is optimised by minimising the photometric error between synthesised images $\hat{\mathcal{I}}$ and captured images $\mathcal{I}$ with camera poses $\Pi$:
\begin{equation}
\mathcal{L}_{rgb}=\sum_{i}^{N}\left\|I_{i}-\hat{I}_{i}\right\|_{2}^{2},
\end{equation}
\begin{equation}
    \Theta^{*} =\arg \min _{\Theta} \mathcal{L}_{rgb}(\hat{\mathcal{I}} \mid \mathcal{I}, \Pi),
\end{equation}
where $\hat{I}_{i}$ is rendered by aggregating radiance colour on camera rays $\mathbf{r}(h)=\mathbf{o}+h \mathbf{d}$ shooting from camera position $\mathbf{o}$ towards direction $\mathbf{d}$:
\begin{equation}
\label{eq:nerf}
    \hat{I}_{i}(\mathbf{r})=\int_{h_{n}}^{h_{f}} T(h) \sigma(\mathbf{r}(h)) \mathbf{c}(\mathbf{r}(h), \mathbf{d}) d h,
\end{equation}
where $h_n$ and $h_f$ defines the near and far bounds along the ray and $T(h)=\exp \left(-\int_{h_{n}}^{h} \sigma(\mathbf{r}(s)) d s\right)$ is the accumulated transmittance along the ray from $h_n$ to $h_f$. \zirui{eq.2 and $\Theta$ is not mentioned anywhere.}


\subsection{Joint Optimisation of Poses and NeRF}
\label{sec: nerfmm}
% As mentioned in the introduction, it is a challenging problem to obtain accurate camera poses robustly in real-world scenes.
We propose to jointly optimise camera poses with NeRF:
%  $\Pi = \{\pi_{i} \mid i=0 \ldots N-1\}$
% When camera poses $\Pi = \{\pi_{i} \mid i=0 \ldots N-1\}$ are not given, they can be parameterised into the NeRF optimisation process and be optimised jointly with the scene representation as:
\begin{equation}
    \Theta^{*}, \Pi^{*}=\arg \min _{\Theta, \Pi} \mathcal{L}_{rgb}(\hat{\mathcal{I}}, \hat{\Pi} \mid \mathcal{I}),
\end{equation}
where $\hat{\Pi}$ denotes the optimising camera poses of input images,
which are initialised as identity transformation at the beginning of joint optimisation.

The camera pose for frame $I_i$ can be expressed as a transformation matrix $\mathbf{T}_i = [\mathbf{R}_i\mid\mathbf{t}_i]$, including rotation $\mathbf{R}_i \in \text{SO}(3)$ and translation $\mathbf{t}_i \in \mathbb{R}^3$. When parameterising into the model as $\pi_i$, we adopt the axis-angle representation $\boldsymbol{\phi}_i \in \mathbb{R}^3$ for rotation and translation $\mathbf{t}$ is still defined in Euclidean space, i.e. $\pi_{i}=(\boldsymbol{\phi}_{i}, \mathbf{t}_{i})$. 

\subsection{Inter-frame Constraint from Pairwise Losses}
\label{sec: nop-nerf}
% \zirui{maybe say inter-frame constraint? pairwise is ambigious, for example, point-point pairwise.}
When poses and geometry are unknown, there are multiple possible radiance fields that can be rendered to training images, with incorrect poses and geometry.
The aforementioned joint optimisation optimises each camera pose independently, which can easily overfit to the target images with incorrect poses. Penalising incorrect estimation of relative poses between frames can help to regularise the joint optimisation towards smooth convergence, especially in a complex camera trajectory.
Therefore, we propose two pairwise losses that constrain relative poses locally.

Specifically, we first generate mono-depth for RGB images using the pretrained mono-depth estimation network (\ie DPT~\cite{ranftl2021vision}),
resulting in $\mathcal{D}= \left\{D_{i} \mid i=0 \ldots N-1 \right\}$.

% the challenges of applying pairwise direclty (distortion)
Note that the estimated mono-depth is distorted by an unknown scale and shift,
and more importantly, the distortion parameters are not consistent over images.
To address the issue, we propose a distortion model $F_{\Psi}: \mathcal{D} \rightarrow \mathcal{D}^{*}$,
where $\Psi = \{\psi_{i} \mid i=0 \ldots N-1\}$ are distortion parameters and optimised individually for all images.
$\psi_{i}$ consists of a scale factor $\alpha_{i}$ and a shift $\beta_{i}$.
Based on the above, the depth map can be undistorted through the linear transformation as
\begin{equation}
\label{eq:depth_w_distort}
    D^{*}_{i} = \alpha_{i} D_{i} + \beta_{i}.
\end{equation}
We expect the undistorted $\mathcal{D}^{*}$ to be multi-view consistent\footnote{This is constrained in Eqn.\eqref{eqn:loss-depth}},
and we leverage it for pose optimisation. 
Similar to per-frame pose optimisation, 
the proposed per-frame distortion optimisation is also jointly learned within NeRF.


% Given that pose optimisation with only the RGB loss can easily fall into local minimum for complex pose trajectory, we propose to add a pairwise loss for relative poses to provide better supervision.
% As free depth maps $\mathcal{D}= \left\{D_{i} \mid i=0 \ldots N-1 \right\}$ can be obtained from a mono-depth estimation network (e.g. DPT~\cite{ranftl2021vision}),
% we can estimate relative poses by matching two point clouds reconstructed from the depth maps. 
% However, due to the ambiguity of mono-depth estimation, the point clouds can have different distortions. 
% Matching the distorted point clouds directly can lead to erroneous results. 
% We propose to parameterise the distortions and optimise jointly with the NeRF model to gain multi-view consistency.

% Writing the transformation to recover the distortion as $F_{\Psi}: \mathcal{D} \rightarrow \mathcal{D}^{*}$, we want to optimise independent distortion parameters for every frame, i.e. $\Psi = \{\psi_{i} \mid i=0 \ldots N-1\}$. As the mono-depth is trained with a scale-shift-invariant loss in DPT, $\psi_{i}$ can be approximated by a scale factor $\alpha_{i}$ and a shift $\beta_{i}$. The depth map can be recovered through the linear transformation as
% $D^{*}_{i} = \alpha_{i} D_{i} + \beta_{i}$.

With the undistorted depth maps $\mathcal{D}^*$, 
we convert them to point clouds $\mathcal{P}^*= \left\{P^*_{i} \mid i=0 \ldots N-1 \right\}$ and optimise the relative pose of sampled image pairs by minimising Chamfer distance.
\begin{equation}
    \label{eq: CD}
    CD({P_{i}}, {P_{j}}) = \sum_{p_{i} \in P_{i}} \min_{p_{j} \in P_{j}} \|p_{i}-p_{j} \|^2_2 + \sum_{p_{j} \in P_{j}} \min_{p_{i} \in P_{i}} \|p_{i}-p_{j} \|^2_2
\end{equation}

The point cloud loss $\mathcal{L}_{pc}$ is formed by sampling consecutive images $(i, j)\in \mathcal{H}$ in a video sequence and computing the Chamfer distance between each image pair:
\begin{equation}
    \mathcal{L}_{pc} = \sum_{(i,j) \in \mathcal{H}}CD(P^{*}_{j}, \mathbf{T}_{j} \mathbf{T}_{i}^{-1}{P^{*}_{i}})
\end{equation}
where the relative pose $\mathbf{T}_{i, j} = \mathbf{T}_{j}\mathbf{T}_{i}^{-1}$ represents the transformation from point cloud $P^{*}_i$ to $P^{*}_j$.

The camera parameters $\Pi$ and distortion parameters $\Psi$ are optimised together with $\mathcal{L}_{pc}$ as
\begin{equation}
     \Pi^{*}, \Psi^{*}=\arg \min _{\Theta, \Pi, \Psi} \mathcal{L}_{pc}(\hat{\Pi}, \hat{\Psi} \mid \mathcal{D})
\end{equation}
Apart from the geometry loss, we add a surface-based photometric loss for each sampled pair, 
which measures the difference between colour of point cloud $P_i^*$ on image $I_i$ and the colour of its projection on image $I_j$:
\begin{equation}
    \mathcal{L}_{rgb-s} = \sum_{(i,j) \in \mathcal{H}}\sum_{(P^{*}_{j}, P^{*}_{j}) \in \mathcal{K}} \| I_{i}(P^{*}_{i}) -I_{j}(\mathbf{T}_{j} \mathbf{T}_{i}^{-1}{P^{*}_{i}})\|^{2}_2
\end{equation}
\begin{equation}
     \Pi^{*}, \Psi^{*}=\arg \min _{\Theta, \Pi, \Psi} \mathcal{L}_{rgb-s}(\hat{\Pi}, \hat{\Psi} \mid \mathcal{D}, \mathcal{I})
\end{equation}

\subsection{Overall Training Pipeline}
% \zirui{maybe just say overall training pipeline.}
% When supervising with mono-depth maps, scale-invariant or scale-shift invariant losses~\cite{eigen2014depth, ranftl2021vision} are often used to address the scale ambiguity.
% In contrast, we incorporate the depth distortion model into NeRF optimisation and compute the los

In addition to constraining pose, the mono-depth also regularises geometry. The depth rendered from NeRF ($\hat{\mathcal{D}}$) is computed as:
\begin{equation}
    \hat{D}_{i}(\mathbf{r})=\int_{h_{n}}^{h_{f}} T(h) \sigma(\mathbf{r}(h)) d h.
\end{equation}
We minimise the discrepancy between the undistorted depth $\mathcal{D}^*$ (as defined in~\cref{eq:depth_w_distort}) and NeRF-rendered depth $\hat{\mathcal{D}}$ for all frames:
\begin{equation}
\label{eqn:loss-depth}
    \mathcal{L}_{depth} = \sum_{i}^{N}\left\|D_{i}^{*}-\hat{D}_{i}\right\|
\end{equation}
As $\hat{\mathcal{D}_i}$ is inherently multi-view consistent, it also provides a global constraint to the depth distortion to encourage learning consistent scales and shifts across views.

During training, the depth loss propagates gradients to not only NeRF parameters $\Theta$ and camera pose $\pi_{i}$, but also distortion parameter $\psi_{i}$, \ie
\begin{equation}
    \Theta^{*}, \Pi^{*}, \Psi^{*}=\arg \min _{\Theta, \Pi, \Psi} \mathcal{L}(\hat{\mathcal{D}}, \hat{\Pi}, \hat{\Psi} \mid \mathcal{D})
\end{equation}
The overall loss function is:
\begin{equation}
\label{eq: 4terms}
\mathcal{L}=\mathcal{L}_{rgb} + \lambda_{1} \mathcal{L}_{depth} + \lambda_{2} \mathcal{L}_{pc} + \lambda_{3} \mathcal{L}_{rgb-s}
\end{equation}
\begin{equation}
    \Theta^{*}, \Pi^{*}, \Psi^{*}=\arg \min _{\Theta, \Pi, \Psi} \mathcal{L}(\hat{\mathcal{I}},\hat{\mathcal{D}}, \hat{\Pi}, \hat{\Psi} \mid \mathcal{I}, \mathcal{D})
\end{equation}




==> 04_method_v1.tex <==
\begin{figure*}[ht]
    \centering
    \includegraphics[width=\linewidth]{images/icp_nerfmm.pdf}
    \caption{\textbf{Model Overview.} Given a sequence of images and the point clouds reconstructed from their monocular depth estimations, we optimise the camera poses $\left\{\mathbf{T}_{i}\right\}_{i=0}^{N-1}$, NeRF model $F_\theta$ and depth distortion parameters $\left\{(\alpha_i, \beta_i) \right\}_{i=0}^{N-1}$ jointly. For frame $I_i$, we select a reference frame $I_j$ ($I_{i+1}$ in this example) and compute the pairwise losses of the point clouds while recovering their distortions. Meanwhile, we optimise a NeRF model with RGB and depth supervision to reconstruct the 3D scene and constrain the camera poses and distortion parameters globally.
    }
    \label{fig:model}
\end{figure*}

\section{Method}\label{sec:method}
We present \methodname, an end-to-end differentiable method for joint pose estimation and novel view synthesis on a sequence of images with their known camera intrinsic parameters.
The key to our method is a robust optimisation of camera rotation in challenging scenes,
where most existing pose-unknown NeRF methods~\cite{lin2021barf, wang2021nerfmm, jeong2021self} often fail.
To achieve this, we introduce single-image depth prior from a pre-trained monocular depth estimation network,
based on which we propose effective constraints on relative camera poses and scene geometry.
However, as the predicted depth (we call pseudo-depth in this paper) is distorted by unknown scales and shifts,
which makes it non-trivial to use,
we propose to jointly learn the distortion parameters for each depth map in the overall optimisation.
In the following subsections, we first go over the NeRF model and NeRF optimisation with unknown poses in \cref{sec: nerf} and \cref{sec: nerfmm} respectively. 
Then in \cref{sec: nop-nerf}, we show how to constrain relative poses and geometry with pseudo-depth. 
We discuss how to parameterise distorted depth maps into the unknown-pose NeRF model and introduce a pairwise point cloud loss for relative poses estimation. 
Finally, we build \methodname that jointly optimises poses, depth distortions and 3D representation of the scene, 
which achieves robust optimisation of complex pose trajectories. 
An overview of our method is shown in \cref{fig:model}.

\subsection{Neural Radiance Field} \label{sec: nerf}

Neural Radiance Field (NeRF)~\cite{mildenhall2021nerf} represents the scene as $F_\theta: (\mathbf{x}, \mathbf{d}) \rightarrow (\mathbf{c}, \sigma)$, 
which maps a 3D location $x \in \mathbb{R}^3$ and viewing direction $\mathbf{d} \in \mathbb{R}^3$ to radiance colour $\mathbf{c} \in \mathbb{R}^3$ and volume density $\sigma$.
Given the captured RGB images $\mathcal{I} = \left\{I_{i} \mid i=0 \ldots N-1 \right\}$ of a scene with their camera poses $\Pi = \{\pi_{i} \mid i=0 \ldots N-1\}$, which are assumed to be accurate,
% learns an implicit representation of a scene from the captured RGB images $\mathcal{I} = \left\{I_{i} \mid i=0 \ldots N-1 \right\}$ of that,
% where accurate camera poses $\Pi = \{\pi_{i} \mid i=0 \ldots N-1\}$ are assumed to be known.
% Given consecutive RGB images of a scene $\mathcal{I} = \left\{I_{i} \mid i=0 \ldots N-1 \right\}$ and their camera poses $\Pi = \{\pi_{i} \mid i=0 \ldots N-1\}$, Neural Radiance Field (NeRF)~\cite{mildenhall2021nerf} learns an implicit representation of the scene including both appearance and geometry. 
NeRF is optimised by minimising the photometric error between the synthesised images $\hat{\mathcal{I}}$ and the observed images $\mathcal{I}$ with the camera poses $\Pi$:
\begin{equation}
\mathcal{L}_{rgb}=\sum_{i}^{N}\left\|I_{i}-\hat{I}_{i}\right\|_{2}^{2},
\end{equation}
\begin{equation}
    \Theta^{*} =\arg \min _{\Theta} \mathcal{L}_{rgb}(\hat{\mathcal{I}} \mid \mathcal{I}, \Pi),
\end{equation}
where $\hat{I}_{i}$ is rendered by aggregating radiance colour on camera rays $\mathbf{r}(h)=\mathbf{o}+h \mathbf{d}$ shooting from camera position $\mathbf{o}$ towards direction $\mathbf{d}$:
\begin{equation}
\label{eq:nerf}
    \hat{I}_{i}(\mathbf{r})=\int_{h_{n}}^{h_{f}} T(h) \sigma(\mathbf{r}(h)) \mathbf{c}(\mathbf{r}(h), \mathbf{d}) d h,
\end{equation}
where $h_n$ and $h_f$ defines the near and far bounds along the ray and $T(h)=\exp \left(-\int_{h_{n}}^{h} \sigma(\mathbf{r}(s)) d s\right)$ is the accumulated transmittance along the ray from $h_n$ to $h_f$.


\subsection{Joint Optimisation of Poses and NeRF}
\label{sec: nerfmm}
As mentioned in introduction, it is a challenging problem to obtain accurate camera poses robustly in real-world scenes.
In this section, we propose to jointly optimise camera poses with NeRF:
%  $\Pi = \{\pi_{i} \mid i=0 \ldots N-1\}$
% When camera poses $\Pi = \{\pi_{i} \mid i=0 \ldots N-1\}$ are not given, they can be parameterised into the NeRF optimisation process and be optimised jointly with the scene representation as:
\begin{equation}
    \Theta^{*}, \Pi^{*}=\arg \min _{\Theta, \Pi} \mathcal{L}_{rgb}(\hat{\mathcal{I}}, \hat{\Pi} \mid \mathcal{I}),
\end{equation}
where $\hat{\Pi}$ denotes the optimising camera poses of input images,
which are initialised as identity transformation at the beginning of joint optimisation.

The camera pose for frame $I_i$ can be expressed as a transformation matrix $\mathbf{T}_i = [\mathbf{R}_i\mid\mathbf{t}_i]$, including rotation $\mathbf{R}_i \in SO(3)$ and translation $\mathbf{t}_i \in \mathbb{R}^3$. When parameterising into the model as $\pi_i$, we adopt the axis-angle representation $\boldsymbol{\phi}_i \in \mathbb{R}^3$ for rotation and translation $\mathbf{t}$ is still defined in Euclidean space, i.e. $\pi_{i}=(\boldsymbol{\phi}_{i}, \mathbf{t}_{i})$. 

\subsection{Local Constraint from Pairwise Losses}
\label{sec: nop-nerf}
% \wenjing{why do we need local constraints:} 
 When poses and geometry are unknown, there are multiple possible radiance field that can be rendered to training images, with incorrect poses and geometry. 
%  Similar to the \textit{shape-radiance ambiguity} discussed in ~\cite{zhang2020nerf++}, we call it \textit{pose-shape-radiance} ambiguity. Different positional encoding strategies~\cite{chng2022garf, lin2021barf} are proposed to constrain the complexity of the learned radiance field. 
% The reluctance of rotation optimisation. (horse example)

% why pairwise, because smooth convergence
To regularise the aforementioned joint optimisation towards smooth convergence, especially in a complex camera trajectory,
we propose two pairwise losses that constrain pose.
Specifically, we first generate pseudo-depth for RGB images using the pretrained monocular depth estimation network (\ie DPT~\cite{ranftl2021vision}),
resulting in $\mathcal{D}= \left\{D_{i} \mid i=0 \ldots N-1 \right\}$.

% the challenges of applying pairwise direclty (distortion)
Note that the estimated pseudo-depth is distorted by an unknown scale and shift,
and more importantly, the distortion parameters are not consistent over images.
To address the issue, we propose a distortion model $F_{\Psi}: \mathcal{D} \rightarrow \mathcal{D}^{*}$,
where $\Psi = \{\psi_{i} \mid i=0 \ldots N-1\}$ are distortion parameters and optimised individually for all images.
$\psi_{i}$ consists of a scale factor $\alpha_{i}$ and a shift $\beta_{i}$.
Based on the above, the depth map can be undistorted through the linear transformation as
\begin{equation}
\label{eq:depth_w_distort}
    D^{*}_{i} = \alpha_{i} D_{i} + \beta_{i}.
\end{equation}
We expect the undistorted $\mathcal{D}^{*}$ to be multi-view consistent\footnote{This is constrained in Eqn.\eqref{eqn:loss-depth}},
and we leverage it for pose optimisation. 
Similar to per-frame pose optimisation, 
the proposed per-frame distortion optimisation is also jointly learned within NeRF.


% Given that pose optimisation with only the RGB loss can easily fall into local minimum for complex pose trajectory, we propose to add a pairwise loss for relative poses to provides better supervision.
% As free depth maps $\mathcal{D}= \left\{D_{i} \mid i=0 \ldots N-1 \right\}$ can be obtained from a monocular depth estimation network (e.g. DPT~\cite{ranftl2021vision}),
% we can estimate relative poses by matching two point clouds reconstructed from the depth maps. 
% However, due to the ambiguity of monocular depth estimation, the point clouds can have different distortions. 
% Matching the distorted point clouds directly can lead to erroneous results. 
% We propose to parameterise the distortions and optimise jointly with the NeRF model to gain multi-view consistency.

% Writing the transformation to recover the distortion as $F_{\Psi}: \mathcal{D} \rightarrow \mathcal{D}^{*}$, we want to optimise independent distortion parameters for every frame, i.e. $\Psi = \{\psi_{i} \mid i=0 \ldots N-1\}$. As the monocular depth is trained with a scale-shift-invariant loss in DPT, $\psi_{i}$ can be approximated by a scale factor $\alpha_{i}$ and a shift $\beta_{i}$. The depth map can be recovered through the linear transformation as
% $D^{*}_{i} = \alpha_{i} D_{i} + \beta_{i}$.

With the undistorted depth maps $\mathcal{D}^*$, 
we convert them to point clouds $\mathcal{P}^*= \left\{P^*_{i} \mid i=0 \ldots N-1 \right\}$ and optimise the relative pose of sampled image pairs by minimising Chamfer distance.
\begin{equation}
    \label{eq: CD}
    CD({P_{i}}, {P_{j}}) = \sum_{p_{i} \in P_{i}} \min_{p_{j} \in P_{j}} \|p_{i}-p_{j} \|^2_2 + \sum_{p_{j} \in P_{j}} \min_{p_{i} \in P_{i}} \|p_{i}-p_{j} \|^2_2
\end{equation}
For a randomly sampled image pair, \eg frame $i$ and $j$, the relative pose $\mathbf{T}_{i, j} = \mathbf{T}_{j}\mathbf{T}_{i}^{-1}$ represents the transformation from point cloud $P^{*}_i$ to $P^{*}_j$.
% \wenjing{And the correspondence set for point clouds $P^{*}_{i}$ and $P^{*}_{j}$ is defined as $\mathcal{K}$. }
Then our objective can be written as:
\begin{equation}
\label{eq:icploss}
    % E(\pi_{i}, \pi_{j}, \psi_{i}, \psi_{j})
    % =\sum_{(p^{*}_{i}, p^{*}_{j}) \in \mathcal{K}} \| p^{*}_{j} -\mathbf{T}_{j} \mathbf{T}_{i}^{-1}{p^{*}_{i}}\|^{2}\\
    E(\pi_{i}, \pi_{j}, \psi_{i}, \psi_{j}) = CD(P^{*}_{j}, \mathbf{T}_{j} \mathbf{T}_{i}^{-1}{P^{*}_{i}})
\end{equation}
where the camera parameters ($\pi_{i}$ and $\pi_{j}$) and distortion parameters ($\psi_{i}, \psi_{j}$) are optimised together.

The point cloud loss $\mathcal{L}_{pc}$ is formed by sampling consecutive images $(i, j)\in \mathcal{H}$ in a video sequence and computing the error in \cref{eq:icploss}:
\begin{equation}
    \mathcal{L}_{pc} = \sum_{(i,j) \in \mathcal{H}}CD(P^{*}_{j}, \mathbf{T}_{j} \mathbf{T}_{i}^{-1}{P^{*}_{i}})
\end{equation}

Apart from the geometry loss, we add a surface-based photometric loss for each sampled pair, 
which measures the difference between colour of point cloud $P_i^*$ on image $I_i$ and the colour of its projection on image $I_j$:
\begin{equation}
    \mathcal{L}_{rgb-s} = \sum_{(i,j) \in \mathcal{H}}\sum_{(P^{*}_{j}, P^{*}_{j}) \in \mathcal{K}} \| I_{i}(P^{*}_{i}) -I_{j}(\mathbf{T}_{j} \mathbf{T}_{i}^{-1}{P^{*}_{i}})\|^{2}
\end{equation}


\subsection{Global Constraint from NeRF}
% When supervising with monocular depth maps, scale-invariant or scale-shift invariant losses~\cite{eigen2014depth, ranftl2021vision} are often used to address the scale ambiguity.
% In contrast, we incorporate the depth distortion model into NeRF optimisation and compute the los

In addition to constraining pose, the mono depth also plays a role in regularising geometry. A depth loss often appears in NeRF optimisation to constrain geometry. In addition to it, our depth loss also constrains the optimisation of depth distortion parameters and encourages the undistorted depths to be multi-view consistent.
We minimise the discrepancy between the undistorted depth $\mathcal{D}^*$ (as defined in~\cref{eq:depth_w_distort}) and NeRF-rendered depth $\hat{\mathcal{D}}$.
Specifically, $\hat{\mathcal{D}}$ is rendered in NeRF by
\begin{equation}
    \hat{D}_{i}(\mathbf{r})=\int_{h_{n}}^{h_{f}} T(h) \sigma(\mathbf{r}(h)) d h.
\end{equation}
Then we compute the depth discrepancy error as 
% When we correctly recover depth maps $\mathcal{D^*}$, the difference between the depth maps $\mathcal{D^*}$ recovered form distortion and the rendered depths $\hat{\mathcal{D}}$ should be minimised. 
\begin{equation}\label{eqn:loss-depth}
    E_{depth}(\Theta, \pi_{i}, \psi_{i}) = \left\|D_{i}^{*}-\hat{D}_{i}\right\|.
\end{equation}
Then the depth loss for all frames $\mathcal{L}_{depth}$ is:
\begin{equation}
    % \mathcal{L}_{depth} = \sum_{i}^{N}\left\|D_{i}^{*}-\hat{D}_{i}\right\|
    \mathcal{L}_{depth} = \sum_{i}^{N}E_{depth}
\end{equation}
During training, the depth loss propagates gradients to not only NeRF parameters $\Theta$ and camera pose $\pi_{i}$, but also distortion parameter $\psi_{i}$.

The overall loss function is:
\begin{equation}
\label{eq: 4terms}
\mathcal{L}=\mathcal{L}_{rgb} + \lambda_{1} \mathcal{L}_{depth} + \lambda_{2} \mathcal{L}_{pc} + \lambda_{3} \mathcal{L}_{rgb-s}
\end{equation}
\begin{equation}
    \Theta^{*}, \Pi^{*}, \Psi^{*}=\arg \min _{\Theta, \Pi, \Psi} \mathcal{L}(\hat{\mathcal{I}},\hat{\mathcal{D}}, \hat{\Pi}, \hat{\Psi} \mid \mathcal{I}, \mathcal{D})
\end{equation}



